Aplicando diferencias finitas para resolver ecuaciones y sistemas de ecuaciones diferenciales parciales sobre dominios planos irregulares simplemente conexos y no conexos

Using exhaustion method and finite differences a new method to solve system of partial differential equations and is presented. This method allows design algorithm to solve linear and nonlinear systems in irregular domains. Applying this method to solve linear and nonlinear problems with prescribed conditions Dirichlet over two-dimensional irregular domains are analyzed.

==> parte2.tex <==
\section{Resultados num\'{e}ricos}    \label{Resultados}              
               
               En esta secci\'{o}n vamos a mostrar los resultados que se
               obtienen al aplicar el m\'{e}todo de la secci\'{o}n \ref{Metodo} 
               para resolver problemas que involucran ecuaciones diferenciales
               parciales lineales y no lineales sobre diferentes tipos de 
               dominios irregulares.                                                                                                                                    
               
               \subsection{Problema 1: Ecuaci\'{o}n de Laplace}                                                              
                                                      
                Consideremos la ecuaci\'{o}n de Laplace con condiciones de 
                Dirichlet no homog\'{e}neas en la frontera
                \begin{eqnarray}
                 \label{Laplace:eq}
                      \nabla^2 a & = & 0,\hspace*{0.3cm} \text{para} \hspace*{0.3cm} (x,y) \in \Omega , \\
                             a & = & f(x,y),\hspace*{0.3cm} \text{para} \hspace*{0.3cm} (x,y) \in   \partial  \Omega , \nonumber
                \end{eqnarray}    
                donde $a=a(x,y)$, $f(x,y)=cos(x) + cos(y)$, $\Omega$ es un dominio 
                irregular y $\partial  \Omega$ es la frontera de $\Omega$.
                
                \begin{enumerate}
                       \item \label{1} Vamos a resolver este problema usando el
                             m\'{e}todo de la secci\'{o}n \ref{Metodo} sobre
                             \begin{enumerate}
                                   \item[a)] Un tri\'{a}ngulo,  \hspace*{1cm} b) Un pent\'{a}gono, \hspace*{1cm}
                                    c) Una estrella.
                             \end{enumerate}
                             
                        \item \label{2} Luego vamos a resolver el problema usando
                              {\it FlexPDE}, el cual es un sofware que aplica 
                              {\it elemento finito} para resolver ecuaciones 
                              diferenciales parciales.
                       
                       \item Finalmente vamos a comparar las soluciones de los
                             incisos \ref{1} y \ref{2}.
                            
                \end{enumerate}    
                
                De acuerdo al m\'{e}todo descrito en la secci\'{o}n \ref{Metodo},
                primero debemos discretizar $\Omega$ y despu\'{e}s debemos
                discretizar la ecuaci\'{o}n de Laplace junto con la condici\'{o}n
                de frontera dada en (\ref{Laplace:eq}). Para esto denotemos 
                con $u_{i j}$ la soluci\'{o}n aproximada de $a$ en el punto
                $(i \Delta x, j \Delta y) \in \overline {\Omega}$, 
                entonces la discretizaci\'{o}n de la ecuaci\'{o}n de Laplace 
                est\'{a} dada por 
                \begin{equation}
                \label{Laplace:disc}   
                       \displaystyle\frac{u_{i+1 j} - 2 u_{i j} + u_{i-1 j}}{\Delta x^2} + \displaystyle\frac{u_{i j+1} - 2 u_{i j} + u_{i j-1}}{\Delta y^2}  =  0,                       
                \end{equation}                                
                ver por ejemplo \cite{Jwt2}. Mientras 
                \begin{equation}
                \label{Laplace:fron}
                       u_{i j}  =  f (i \Delta x, j \Delta y), \hspace*{0.3cm} \text{para} \hspace*{0.3cm} (i \Delta x, j \Delta y) \in   \partial  \overline {\Omega},
                \end{equation}
                denota la discretizaci\'{o}n de la frontera.
                
                Ya hab\'{i}amos visto en el ejemplo \ref{ejemplo1} de la 
                secci\'{o}n \ref{Metodo} que la discretizaci\'{o}n (\ref{Laplace:disc})
                junto con (\ref{Laplace:fron}) da lugar a un sistema de 
                ecuaciones lineales, mismo que resolveremos aplicando el
                m\'{e}todo iterativo de Gauss-Seidel.
                
                En las tablas \ref{Laplace:tab1} y \ref{Laplace:tab2} 
                podemos observar los resultados de los valores m\'{a}ximos
                y m\'{i}nimos y sus posiciones. Al comparar estos 
                resultados podemos notar que son aproximadamente los
                mismos. Mientras que en la figura \ref{Laplace:fig1} se 
                puede ver la proyecci\'{o}n en el plano $xy$ de cada una 
                de las soluciones obtenidas con {\it Matlab} y con
                {\it FlexPDE} sobre cada uno de los dominios irregulares.                                                      
                                                   
                
                \begin{table}[t!]
                \centering
                \begin{tabular}{|c|c|c|c|c|} %\multirow{2}{1.3cm}{$(0,0,0)$}
                \hline   
                \multirow{4}{1.4cm}{Dominio} & \multicolumn{2}{c|}{\multirow{2}{*}{Matlab}}         & \multicolumn{2}{c|}{\multirow{2}{*}{FlexPDE}}   \\
                &  \multicolumn{2}{c|}{}  & \multicolumn{2}{c|}{}  \\ \cline{2-5}
                                 
                                  
                 
                         & \multirow{2}{2.6cm}{\hspace*{0.6cm} $u_{min}$} 
                         & \multirow{2}{2.6cm}{$(x_{min}, y_{min})$} 
                         & \multirow{2}{2.6cm}{\hspace*{0.6cm} $u_{min}$ } 
                         & \multirow{2}{2.6cm}{$(x_{min}, y_{min})$ }      \\                            
                              &               &   &               &        \\
                 \hline             
                 \hline
                  $a)$ & $-1.6305$  & $(8.68, 9.04)$ & $-1.68$ & $(8.72, 9.01)$  \\
                  $b)$ & $-1.9683$  & $(3.16, 9.48)$ & $-2.00$ & $(3.06, 9.41)$  \\                  
                  $c)$ & $-1.8938$  & $(9.84, 3.20)$ & $-1.91$ & $(9.84, 3.20)$ \\                 
                \hline 
                \end{tabular}
                \caption{Valores m\'{i}nimos y sus coordenadas correspondientes 
                         a las soluciones mostradas en la figura \ref{Laplace:fig1}.} %, \ref{Laplace:fig2}, \ref{Laplace:fig3} y \ref{Laplace:fig4}.}
                \label{Laplace:tab1} 
                \end{table}                                   
                
                
                
                
                \begin{table}[t!]
                \centering
                \begin{tabular}{|c|c|c|c|c|} %\multirow{2}{1.3cm}{$(0,0,0)$}
                \hline
                \multirow{4}{1.4cm}{Dominio} & \multicolumn{2}{c|}{\multirow{2}{*}{Matlab}}           & \multicolumn{2}{c|}{\multirow{2}{*}{FlexPDE}}  \\
                                       &  \multicolumn{2}{c|}{}  & \multicolumn{2}{c|}{}  \\ \cline{2-5} 
                                       
                                       & \multirow{2}{2.6cm}{ \hspace*{0.6cm}  $u_{max}$} 
                                       & \multirow{2}{2.6cm}{$(x_{max}, y_{max})$ } 
                                       & \multirow{2}{2.6cm}{\hspace*{0.6cm} $u_{max}$ }  
                                       & \multirow{2}{2.6cm}{ $(x_{max}, y_{max})$ } \\                
                                       &        &        &        &   \\ \hline
                \hline
                  $a)$  & $1.6877$ & $(7.00, 12.24)$ & $1.70$ & $(6.99, 12.24)$   \\
                  $b)$  & $1.9114$ & $(12.24, 6.32)$ & $1.95$ & $(12.28, 6.44)$   \\                  
                  $c)$  & $1.6882$ & $(7.00, 12.24)$ & $1.70$ & $(6.99, 12.24)$   \\                 
                \hline 
                \end{tabular}
                \caption{Valores m\'{a}ximos y sus coordenadas correspondientes 
                         a las soluciones mostradas en la figura \ref{Laplace:fig1}.}
                \label{Laplace:tab2} 
                \end{table}        
                
                
                \begin{figure}[b]
                \centering
                \begin{tabular}{||c||}
                \hline
                \includegraphics[width=13cm,height=1cm]{imagenes/escala.png} \\                                  
                \hline
                \end{tabular}
                \caption{Espectro de la escala de colores de {\it Matlab} y {\it FlexPDE}.}
                \label{espectro:fig}
                \end{figure}     
                

                \begin{figure}[h!]  
                \centering
                \begin{tabular}{||c  c||}
                \hline                                   
                \includegraphics[width=6.0cm,height=5.5cm]{imagenes/fig2a.jpg} & \includegraphics[width=6.0cm,height=5.5cm]{imagenes/prog2_01.png} \\ %& 
                %\includegraphics[width=4.0cm,height=4.0cm]{imagenes/fig2.jpg} \\ 
                \multicolumn{2}{|| c ||}{ Dominio a) }\\                   
                \includegraphics[width=6.0cm,height=5.5cm]{imagenes/fig3a.jpg} & \includegraphics[width=6.0cm,height=5.5cm]{imagenes/prog3_01.png} \\ %&
                %\includegraphics[width=4.0cm,height=4.0cm]{imagenes/fig3.jpg} \\
                \multicolumn{2}{|| c ||}{ Dominio b) }\\                                              
                \includegraphics[width=6.0cm,height=5.5cm]{imagenes/fig4a.jpg} & \includegraphics[width=6.0cm,height=5.5cm]{imagenes/prog4_01.png} \\ %& 
                %\includegraphics[width=4.0cm,height=4.0cm]{imagenes/fig4.jpg} \\ 
                \multicolumn{2}{|| c ||}{ Dominio c) }\\                                                             
                \hline
                \end{tabular}
                \caption{Soluci\'{o}n num\'{e}rica de la ecuaci\'{o}n (\ref{Laplace:eq})  
                        con {\it Matlab} y con {\it FlexPDE}, a la izquierda y a la derecha,
                        respectivamente.}  
                \label{Laplace:fig1} 
                \end{figure} 
                
                
                En la secci\'{o}n \ref{Metodo} ya hab\'{i}amos mencionado que 
                para la graficar las soluciones en {\it Matlab} ibamos a estar
                ocupando la escala del espectro de colores donde el color rojo
                representa el valor m\'{a}s alto y el azul representa el valor
                m\'{i}nimo. Adem\'{a}s de esta escala de colores tambi\'{e}n 
                vamos a usar la escala del espectro de colores de {\it FlexPDE} 
                en donde el color rojo tambi\'{e}n se utiliza para representar
                el valor m\'{a}s alto, mientras que el color morado se usa para 
                representar el valor menor. En la figura \ref{espectro:fig} se
                pueden observar ambas escalas de colores las cuales ser\'{a}n 
                utilizadas de aqu\'{i} en adelante.
                
                                                   
\newpage                
                
               
               \subsection{Problema 2: Ecuaci\'{o}n de Poisson}
                                                                                    
                Consideremos la ecuaci\'{o}n de Poisson con condiciones de 
                Dirichlet no homog\'{e}neas en la frontera
                \begin{eqnarray}
                 \label{Poisson:eq}
                      -\nabla^2 a & = & f(x,y),\hspace*{0.3cm}\text{para}\hspace*{0.3cm} (x,y)\in\Omega, \\
                             a & = & g(x,y),\hspace*{0.3cm} \text{para} \hspace*{0.3cm} (x,y) \in   \partial  \Omega , \nonumber
                \end{eqnarray}    
                donde $a=a(x,y)$, $f(x,y)=-1$, $g(x,y)=1$, $\Omega$ es un dominio irregular y
                $\partial  \Omega$ es la frontera de $\Omega$.   
                
                
                \begin{enumerate}
                       \item \label{1} Vamos a resolver este problema usando el
                             m\'{e}todo de la secci\'{o}n \ref{Metodo} sobre
                             los siguientes dominios
                             \begin{enumerate}
                                   \item[d)] el dominio determinado entre dos rect\'{a}ngulos,
                                             uno inscrito en el otro,
                                   \item[e)] el dominio determinado entre un rect\'{a}ngulo y
                                             una estrella inscrita en el,
                                   \item[f)] el dominio determinado entre dos estrellas, una 
                                              inscrita en la otra.
                             \end{enumerate}
                             
                        \item \label{2} Luego vamos a resolver el mismo problema usando
                              {\it FlexPDE}.
                       
                       \item Finalmente vamos a comparar las soluciones de los
                             incisos \ref{1} y \ref{2}.
                            
                \end{enumerate} 
                
                Al igual que en el problema anterior, primero discretizamos 
                cada uno de los dominios y despu\'{e}s discretizamos el 
                problema (\ref{Poisson:eq}). Para esto denotemos con $u_{i j}$ 
                la soluci\'{o}n aproximada de $a$ en el punto
                $(i \Delta x, j \Delta y) \in \overline {\Omega}$, entonces
                la discretizaci\'{o}n de la ecuaci\'{o}n de Poisson est\'{a} 
                dada por
                \begin{equation}
                \label{Poisson:dis}   
                       \displaystyle\frac{u_{i+1 j} - 2 u_{i j} + u_{i-1 j}}{\Delta x^2} + \displaystyle\frac{u_{i j+1} - 2 u_{i j} + u_{i j-1}}{\Delta y^2}  =  f(i \Delta x, j \Delta y),                       
                \end{equation}                                
                ver por ejemplo \cite{Jwt2}. Mientras 
                \begin{equation}
                \label{Poisson:fron}
                       u_{i j}  =  g (i \Delta x, j \Delta y), \hspace*{0.3cm} \text{para} \hspace*{0.3cm} (i \Delta x, j \Delta y) \in   \partial  \overline {\Omega},
                \end{equation}
                denota la discretizaci\'{o}n de la frontera.                                
                                
                Para resolver el sistema de ecuaciones lineales (\ref{Poisson:dis})
                junto con (\ref{Poisson:fron}) sobre cada uno de los diminios
                irregulares aplicamos el m\'{e}todo iterativo de Jacobi.
                
                En las tablas \ref{Poisson:tab1} y \ref{Poisson:tab2} se muestran 
                los valores m\'{a}ximos y m\'{i}nimos y su localizaci\'{o}n que
                obtuvimos en {\it Matlab} y {\it FlexPDE}. Mientras que las 
                proyecciones de las soluciones sobre el plano $xy$ que obtuvimos
                en {\it Matlab} y {\it FlexPDE} se ilustran a la izquierda 
                y a la derecha de la figura \ref{Poisson:fig1}, respectivamente.
                                                                              
                
                 
                
                \begin{table}[t!]
                \centering
                \begin{tabular}{|c|c|c|c|c|} %\multirow{2}{1.3cm}{$(0,0,0)$}
                \hline   
                \multirow{4}{1.4cm}{Dominio} & \multicolumn{2}{c|}{\multirow{2}{*}{Matlab}}         & \multicolumn{2}{c|}{\multirow{2}{*}{FlexPDE}}   \\
                &  \multicolumn{2}{c|}{}  & \multicolumn{2}{c|}{}  \\ \cline{2-5}                                                                                    
                         & \multirow{2}{2.6cm}{\hspace*{0.6cm} $u_{min}$} 
                         & \multirow{2}{2.6cm}{$(x_{min}, y_{min})$} 
                         & \multirow{2}{2.6cm}{\hspace*{0.6cm} $u_{min}$ } 
                         & \multirow{2}{2.6cm}{$(x_{min}, y_{min})$ }      \\                            
                              &               &   &               &        \\
                \hline             
                \hline
                \multirow{4}{0.4cm}{$d)$} & \multirow{4}{1.1cm}{$1.0013$} & $(1.0200,  8.9800)$ & \multirow{4}{0.8cm}{$1.00$} & \multirow{4}{2.1cm}{$(12.00, 9.00)$}  \\
                       &           & $(11.9800, 8.9800)$ &        &                  \\
                       &           & $(11.9800, 1.0200)$ &        &                  \\
                       &           & $( 1.0200, 1.0200)$ &        &                  \\
                \hline
                  $e)$ & $1.0013$  & $(11.9800, 8.9800)$ & $1.00$ & $(12.00, 1.00)$  \\
                \hline
                  $f)$ & $1.0002$  & $(10.4800, 1.0200)$ & $1.00$ & $(1.00,8.00)$ \\                 
                \hline 
                \end{tabular}
                \caption{Valores m\'{i}nimos y sus coordenadas correspondientes 
                         a las soluciones mostradas en la figura \ref{Poisson:fig1}.}
                \label{Poisson:tab1} 
                \end{table}                                   
                                                
                
                \begin{table}[t!]
                \centering
                \begin{tabular}{|c|c|c|c|c|} %\multirow{2}{1.3cm}{$(0,0,0)$}
                \hline
                \multirow{4}{1.4cm}{Dominio} & \multicolumn{2}{c|}{\multirow{2}{*}{Matlab}}           & \multicolumn{2}{c|}{\multirow{2}{*}{FlexPDE}}  \\
                                       &  \multicolumn{2}{c|}{}  & \multicolumn{2}{c|}{}  \\ \cline{2-5}                                        
                                       & \multirow{2}{2.6cm}{ \hspace*{0.6cm}  $u_{max}$} 
                                       & \multirow{2}{2.6cm}{$(x_{max}, y_{max})$ } 
                                       & \multirow{2}{2.6cm}{\hspace*{0.6cm} $u_{max}$ }  
                                       & \multirow{2}{2.6cm}{ $(x_{max}, y_{max})$ } \\                
                                       &        &        &        &   \\ \hline
                \hline
                  \multirow{2}{0.4cm}{$d)$}  & \multirow{2}{1.1cm}{$2.5370$} & $(2.7800, 5.0000)$  & \multirow{2}{0.8cm}{$2.54$} & \multirow{2}{2cm}{$(2.75, 5.00)$}  \\
                        &          & $(10.2200, 5.0000)$ &        &                  \\
                \hline      
                  $e)$  & $2.7362$ & $(3.0400, 3.8800)$  & $2.73$ & $(3.09, 3.82)$   \\ 
                \hline
                  $f)$  & $1.5954$ & $(7.0000, 8.2800)$  & $1.58$ & $(7.00, 8.28)$   \\                 
                \hline 
                \end{tabular}
                \caption{Valores m\'{a}ximos y sus coordenadas correspondientes 
                         a las soluciones mostradas en la figura \ref{Poisson:fig1}.}
                \label{Poisson:tab2} 
                \end{table}           
                
                
                \begin{figure}[h!]  
                \centering
                \begin{tabular}{||c  c||}
                \hline                                   
                \includegraphics[width=6.0cm,height=5.5cm]{imagenes/fig5a.jpg} & \includegraphics[width=6.0cm,height=5.5cm]{imagenes/prog5_01.png} \\ %& 
                %\includegraphics[width=4.0cm,height=4.0cm]{imagenes/fig2.jpg} \\ 
                \multicolumn{2}{|| c ||}{ Dominio d) }\\                   
                \includegraphics[width=6.0cm,height=5.5cm]{imagenes/fig6a.jpg} & \includegraphics[width=6.0cm,height=5.5cm]{imagenes/prog6_01.png} \\ %&
                %\includegraphics[width=4.0cm,height=4.0cm]{imagenes/fig3.jpg} \\
                \multicolumn{2}{|| c ||}{ Dominio e) }\\                                              
                \includegraphics[width=6.0cm,height=5.5cm]{imagenes/fig7a.jpg} & \includegraphics[width=6.0cm,height=5.5cm]{imagenes/prog7_01.png} \\ %& 
                %\includegraphics[width=4.0cm,height=4.0cm]{imagenes/fig4.jpg} \\ 
                \multicolumn{2}{|| c ||}{ Dominio f) }\\                                                             
                \hline
                \end{tabular}
                \caption{Soluci\'{o}n num\'{e}rica de la ecuaci\'{o}n (\ref{Poisson:eq})  
                        sobre diferentes dominios irregulares.}  
                \label{Poisson:fig1} 
                \end{figure} 
                
\newpage                
                
                \subsection{Problema 3: Ecuaci\'{o}n de Helmholtz} 
                                                      
               Consideremos el siguiente problema
                \begin{eqnarray}
                 \label{Helmholtz:eq}
                      \Delta a + f(x,y)a & = & g(x,y),\hspace*{0.3cm}\text{para}\hspace*{0.3cm} (x,y)\in\Omega,\\ 
                      a & = & h(x,y),\hspace*{0.3cm} \text{para} \hspace*{0.3cm} (x,y) \in \partial \Omega , \nonumber
                \end{eqnarray}    
                donde $a=a(x,y)$, $f(x,y)=$, $g(x,y)=$, $h(x,y)=$, $\Omega$ es una regi\'{o}n irregular y
                $\partial  \Omega$ es la frontera de $\Omega$.                                   
                
                \begin{enumerate}
                       \item \label{1} Vamos a resolver este problema usando el
                             m\'{e}todo de la secci\'{o}n \ref{Metodo} sobre
                             \begin{enumerate}[leftmargin=2.7cm]
                                    \item[g)] Un sector circular, \hspace*{1.0cm}  h) Hipocicloide, 
                                    
                                     \hspace*{1.0cm} i) Una flor de cuatro p\'{e}talos.
                             \end{enumerate}
                             
                        \item \label{2} Luego vamos a resolver el problema usando
                              {\it FlexPDE}.
                       
                       \item Finalmente vamos a comparar las soluciones de los
                             incisos \ref{1} y \ref{2}.
                            
                \end{enumerate} 
                
                Al igual que en los problemas anteriores vamos a resolver 
                num\'{e}ricamente este problema. Para esto primero discretizamos
                cada una de los dominios dados y despu\'{e}s discretizamos 
                la ecuac\'{i}on diferencial parcial. Denotemos con $u_{i j}$ 
                la soluci\'{o}n aproximada de $a$ en el punto
                $(i \Delta x, j \Delta y) \in \overline {\Omega}$, entonces
                la discretizaci\'{o}n de la ecuaci\'{o}n de Helmholtz est\'{a} 
                dada por
                \begin{equation}
                \label{Helmholtz:dis}   
                       \displaystyle\frac{u_{i+1 j} - 2 u_{i j} + u_{i-1 j}}{\Delta x^2} + \displaystyle\frac{u_{i j+1} - 2 u_{i j} + u_{i j-1}}{\Delta y^2}  =  f(i \Delta x, j \Delta y),                       
                \end{equation}                                
                ver por ejemplo \cite{Jwt2}. Mientras 
                \begin{equation}
                \label{Helmholtz:fron}
                       u_{i j}  =  g (i \Delta x, j \Delta y), \hspace*{0.3cm} \text{para} \hspace*{0.3cm} (i \Delta x, j \Delta y) \in   \partial  \overline {\Omega},
                \end{equation}
                denota la discretizaci\'{o}n de la frontera.  
                
\newpage                
                               
               \subsection{Problema no lineal: Estado estacionario de los PP} 
               
                Consideremos el siguiente sistema de ecuaciones no lineales 
                que describe el estado estacionario de la interacci\'{o}n 
                entre polinizadores y plantas                
                \begin{eqnarray}
                 \label{eq:eq1numre}
                      D_1 div \left[ f_1(p) \bigtriangledown a \right] + a(k-a) + \displaystyle\frac{ap}{1+p} & = & 0, \\
                      - \displaystyle\frac{1}{2} p + \displaystyle\frac{ap}{1+p}   & = &  0,  \nonumber
                \end{eqnarray}                
                con condiciones de Dirichlet no homog\'{e}neas, esto es
                \begin{equation}
                 a(x,y) = a_f, \hspace{0.2cm} p(x,y) = p_f, \hspace{0.5cm} \forall (x,y) \in \partial \Omega,
                \end{equation}
                donde $a=a(x,y)$ y $p=p(x,y)$ representan la densidad de 
                los polinizadores y las plantas, respectivamente, en el 
                punto $(x,y)$; $a_f$ y $p_f$ son constantes positivas. 
                N\'{o}tese que el sistema (\ref{eq:eq1numre}) puede ser un
                sistema degenerado, lo cual depender\'{a} de los valores 
                de $f_1(p)$.   
                
                \begin{enumerate}
                       \item \label{1} Vamos a resolver este problema usando el
                             m\'{e}todo de la secci\'{o}n \ref{Metodo} sobre
                             \begin{enumerate} [leftmargin=1.8cm]
                                    \item[j)] El Distrito Federal, \hspace*{1.0cm} 
                                         k) Puebla, \hspace*{1.0cm} l) M\'{e}xico.
                             \end{enumerate}
                             Para este prop\'{o}sito vamos a considerar $k=0.45$, 
                             $a_f= 0.8851$, $p_f= 0.7702$ y dos casos particulares
                             de $f_1$: $f_1(p)=1$ y $f_1(p)=p$.
                             
                        \item \label{2} Luego vamos a resolver el problema usando
                              {\it FlexPDE}.
                       
                       \item Despu\'{e}s vamos a comparar las soluciones de los
                             incisos \ref{1} y \ref{2}.
                             
                       \item Finalmente vamos a rehacer los incisos anteriores 
                             considerando los valores $a_f= 0.8851$, $p_f= 0.7702$.
                            
                \end{enumerate}                                                 
                
                Con el prop\'{o}sito de buscar soluciones no constantes 
                para el sistema (\ref{eq:eq1numre}) consideremos que $p \neq 0$, 
                as\'{i} de la segunda ecuaci\'{o}n de este sistema se 
                sigue que
                \begin{equation}
                \label{eq:solp}  
                         p= 2a-1,
                \end{equation} 
                la cual nos est\'{a} diciendo que la distribuci\'{o}n final
                de la poblaci\'{o}n de las plantas est\'{a} directamente 
                relacionada con la distribuci\'{o}n final de la poblaci\'{o}n 
                de los polinizadores.
                
                Al sustituir la expresi\'{o}n (\ref{eq:solp}) en la parte no  
                lineal de la primera ecuaci\'{o}n del sistema (\ref{eq:eq1numre})  
                obtenemos
                \begin{equation}    
                 \label{eq:genpp}            
                      D_1 div \left[ f_1(p) \bigtriangledown a \right] -a^2 + a(k+1) -\displaystyle\frac{1}{2} =  0.
                \end{equation}               
                Ahora consideremos las siguientes aproximaciones                                  
                \begin{equation}
                \label{pp:aprox}
                \begin{array}{cccccc}
                       (a_{x})_{ij}     & \approx  & \displaystyle\frac{u_{i+\frac{1}{2} j} - u_{i-\frac{1}{2} j}}{\Delta x}, &
                       (a_{y})_{ij}    & \approx  & \displaystyle\frac{u_{i j+\frac{1}{2}} - u_{i j-\frac{1}{2}}}{\Delta y},                          
                \end{array}                                         
                \end{equation}                
                donde $u_{i j}$ y $p_{i j}$ denota la soluci\'{o}n aproximada de $a$ 
                y $p$ en el punto $(i \Delta x, j \Delta y)$. 
                                
                Al aplicar las expresiones anteriores para aproximar la ecuaci\'{o}n
                diferencial (\ref{eq:genpp}) en el punto $(i \Delta x, j \Delta y)$
                obtenemos el siguiente esquema de ecuaciones no lineales                 
                \begin{equation}
                \label{eq:disc}                
                 D_1 \left [ \displaystyle\frac{c_{ij}}{\Delta x^2} + \displaystyle\frac{d_{ij}}{\Delta y^2} \right ] - u_{i j}^2 + u_{i j}(k+1) - \displaystyle\frac{1}{2} =0, 
                \end{equation}
                donde
                \begin{eqnarray*}                                 
                 c_{ij} & = & f_1(p_{i j}) u_{i+1 j} - 2 f_1(p_{i j}) u_{i j} + f_1( p_{i j})u_{i-1 j}, \\
                 d_{ij} & = & f_1(p_{i j}) u_{i j+1} - 2 f_1(p_{i j}) u_{i j} + f_1(p_{i j})u_{i j-1}                                  
                \end{eqnarray*}
                con $f_1(p)=1$ \'{o} $f_1(p)=p$.                                                                
                 
                Ahora bien, para resolver este sistema de ecuaciones no lineales (\ref{eq:disc}) 
                sobre cada dominio irregular, aplicamos el m\'{e}todo iterativo de 
                punto fijo. 
                                                                                                
                
                \begin{table}[t!]
                \centering
                \begin{tabular}{|c|c|c|c|c|} %\multirow{2}{1.3cm}{$(0,0,0)$}
                \hline
                \multirow{4}{1.4cm}{Dominio} & \multicolumn{2}{c|}{\multirow{2}{*}{Matlab}}           & \multicolumn{2}{c|}{\multirow{2}{*}{FlexPDE}}  \\
                                       &  \multicolumn{2}{c|}{}  & \multicolumn{2}{c|}{}  \\ \cline{2-5} 
                                       
                                       & \multirow{2}{2.6cm}{ \hspace*{0.6cm}  $u_{max}$} 
                                       & \multirow{2}{2.6cm}{$(x_{max}, y_{max})$ } 
                                       & \multirow{2}{2.6cm}{\hspace*{0.6cm} $u_{max}$ }  
                                       & \multirow{2}{2.6cm}{ $(x_{max}, y_{max})$ } \\                
                                       &        &        &        &   \\ \hline
                \hline
                  $j)$  & $0.7321$ & $(7.28, 8.08)$ & $0.73$  & $(7.30, 7.97)$   \\
                  $k)$  & $0.7278$ & $(8.68, 9.16)$ & $0.726$ & $(8.62, 9.15)$   \\                  
                  $l)$  & $0.7014$ & $(9.36, 7.04)$ & $0.701$ & $(9.25, 7.22)$   \\                 
                \hline 
                \end{tabular}
                \caption{Concentraci\'{o}n m\'{a}xima de la densidad de los polinizadores y 
                         sus coordenadas correspondientes a las soluciones mostradas
                         en las figuras \ref{pol:fig1}, \ref{pol:fig2}, \ref{pol:fig3},
                         \ref{pol:fig4}, \ref{pol:fig5} y \ref{pol:fig6}.}
                \label{pol:tab1} 
                \end{table}  
                
                \begin{table}[t!]
                \centering
                \begin{tabular}{|c|c|c|c|c|} %\multirow{2}{1.3cm}{$(0,0,0)$}
                \hline
                \multirow{4}{1.4cm}{Dominio} & \multicolumn{2}{c|}{\multirow{2}{*}{Matlab}}           & \multicolumn{2}{c|}{\multirow{2}{*}{FlexPDE}}  \\
                                       &  \multicolumn{2}{c|}{}  & \multicolumn{2}{c|}{}  \\ \cline{2-5} 
                                       
                                       & \multirow{2}{2.6cm}{ \hspace*{0.6cm}  $v_{max}$} 
                                       & \multirow{2}{2.6cm}{$(x_{max}, y_{max})$ } 
                                       & \multirow{2}{2.6cm}{\hspace*{0.6cm} $v_{max}$ }  
                                       & \multirow{2}{2.6cm}{ $(x_{max}, y_{max})$ } \\                
                                       &        &        &        &   \\ \hline
                \hline
                  $j)$  & $0.4642$ & $(7.28, 8.08)$ & $0.46$  & $(7.30, 7.97)$   \\
                  $k)$  & $0.4557$ & $(8.68, 9.16)$ & $0.45$  & $(8.62, 9.15)$   \\                  
                  $l)$  & $0.4027$ & $(9.36, 7.04)$ & $0.403$ & $(9.25, 7.22)$   \\                 
                \hline 
                \end{tabular}
                \caption{Concentraci\'{o}n m\'{a}xima de la densidad de las plantas y  
                         sus coordenadas correspondientes a las soluciones mostradas
                         en las figuras \ref{pol:fig1}, \ref{pol:fig2}, \ref{pol:fig3},
                         \ref{pol:fig4}, \ref{pol:fig5} y \ref{pol:fig6}.}
                \label{pol:tab2} 
                \end{table}
                
                
                En las tablas \ref{pol:tab1} y \ref{pol:tab2} se resumen algunos
                resultados que obtuvimos, en \'{e}stas podemos observar que los 
                valores obtenidos con {\it Matlab} son aproximadamente los mismos
                valores que los obtenidos con {\it FlexPDE}.
                
                Adem\'{a}s, en las figuras \ref{pol:fig1}, \ref{pol:fig2}, 
                \ref{pol:fig3}, \ref{pol:fig4}, \ref{pol:fig5} y \ref{pol:fig6}
                se pueden ver las gr\'{a}ficas de las soluciones y sus 
                proyecciones en el plano $xy$ que se obtuvieron con {\it Matlab}
                y con {\it FlexPDE}. En \'{e}stas podemos observar que las 
                soluciones son cualitativamente las mismas. Por otro lado, 
                estos resultados se pueden interpretar de la siguiente manera.
                
                En la gr\'{a}fica de la distribuci\'{o}n de los polinizadores 
                y las plantas podemos apreciar que en cada dominio 
                \begin{enumerate}
                      \item Para el primer par de valores de frontera
                      
                            \begin{enumerate}
                                  \item las dos poblaciones se concentran en el 
                                        interior del dominio,
                                  \item el lugar donde hay mayor concentraci\'{o}n 
                                        de las dos poblaciones coincide,
                            \end{enumerate}
                            es decir las problaciones coexisten
                 
                 
                      \item Para el segundo par de valores de frontera
                      
                            \begin{enumerate}
                                  \item las dos poblaciones se repliegan hacia 
                                        la frontera del dominio,
                                  \item el lugar donde parece que se concentraci\'{o}n 
                                        de las dos poblaciones es la frontera,
                            \end{enumerate}
                            es decir las problaciones coexisten
                      
                \end{enumerate}

                De hecho al variar continuamente las condiciones de frontera 
                de manera adecuada, observamos que cuando las soluciones cambian
                de convexas a concavas se obtiene el estado estacionario positivo 
                y homog\'{e}neo
                \begin{equation}
                     a(x,y)=a^*, \hspace*{0.5cm} p(x,y)=p^*.
                \end{equation}
                donde $a^*$ y $p^*$ es el punto de equilibrio del sistema 
                que modela la din\'{a}mica temporal de los polinizadores  
                y las plantas.


                
                
                \begin{figure}[h!]
                \centering
                \begin{tabular}{||c|c||}
                \hline
                \verb+ POLINIZADORES + & \verb+ PLANTAS  + \\ \hline
                \includegraphics[width=4.8cm,height=4.2cm]{imagenes/fig8pp2a.jpg} & \includegraphics[width=4.8cm,height=4.2cm]{imagenes/fig8pp2b.jpg}  \\  
                \hline
                \includegraphics[width=4.8cm,height=4.2cm]{imagenes/fig8pp1a.jpg} & \includegraphics[width=4.8cm,height=4.2cm]{imagenes/fig8pp1b.jpg} \\ 
                \hline                               
                \end{tabular}
                \caption{Estado estacionario del sistema (\ref{eq:eq1numre}) con $D_1=10$.}
                \label{pol:fig1} 
                \end{figure}      


                \begin{figure}[h!]
                \centering
                \begin{tabular}{||c|c||}
                \hline
                \verb+ POLINIZADORES + & \verb+ PLANTAS  + \\ \hline
                \includegraphics[width=4.8cm,height=4.2cm]{imagenes/prog8_03.png} & \includegraphics[width=4.8cm,height=4.2cm]{imagenes/prog8_04.png}  \\  
                \hline
                \includegraphics[width=4.8cm,height=4.2cm]{imagenes/prog8_01.png} & \includegraphics[width=4.8cm,height=4.2cm]{imagenes/prog8_02.png} \\ 
                \hline
                \end{tabular}
                \caption{Estado estacionario del sistema (\ref{eq:eq1numre}) con $D_1=10$.}
                \label{pol:fig2} 
                \end{figure}  
                
                
                 \begin{figure}[h!]
                \centering
                \begin{tabular}{||c|c||}
                \hline
                \verb+ POLINIZADORES + & \verb+ PLANTAS  + \\ \hline
                \includegraphics[width=4.8cm,height=4.2cm]{imagenes/fig9pp2a.jpg} & \includegraphics[width=4.8cm,height=4.2cm]{imagenes/fig9pp2b.jpg}  \\  
                \hline
                \includegraphics[width=4.8cm,height=4.2cm]{imagenes/fig9pp1a.jpg} & \includegraphics[width=4.8cm,height=4.2cm]{imagenes/fig9pp1b.jpg} \\ 
                \hline  
                \end{tabular}
                \caption{Estado estacionario del sistema (\ref{eq:eq1numre}) con $D_1=10$.}
                \label{pol:fig3} 
                \end{figure}      


                \begin{figure}[h!]
                \centering
                \begin{tabular}{||c|c||}
                \hline
                \verb+ POLINIZADORES + & \verb+ PLANTAS  + \\ \hline
                \includegraphics[width=4.8cm,height=4.2cm]{imagenes/prog9_03.png} & \includegraphics[width=4.8cm,height=4.2cm]{imagenes/prog9_04.png}  \\  
                \hline
                \includegraphics[width=4.8cm,height=4.2cm]{imagenes/prog9_01.png} & \includegraphics[width=4.8cm,height=4.2cm]{imagenes/prog9_02.png} \\ 
                \hline
                \end{tabular}
                \caption{Estado estacionario del sistema (\ref{eq:eq1numre}) con $D_1=10$.}
                \label{pol:fig4} 
                \end{figure}  
                
                
                 \begin{figure}[h!]
                \centering
                \begin{tabular}{||c|c||}
                \hline
                \verb+ POLINIZADORES + & \verb+ PLANTAS  + \\ \hline
                \includegraphics[width=4.8cm,height=4.2cm]{imagenes/fig10pp2a.jpg} & \includegraphics[width=4.8cm,height=4.2cm]{imagenes/fig10pp2b.jpg}  \\  
                \hline
                \includegraphics[width=4.8cm,height=4.2cm]{imagenes/fig10pp1a.jpg} & \includegraphics[width=4.8cm,height=4.2cm]{imagenes/fig10pp1b.jpg} \\ 
                \hline  
                \end{tabular}
                \caption{Estado estacionario del sistema (\ref{eq:eq1numre}) con $D_1=10$.}
                \label{pol:fig5} 
                \end{figure}      


                \begin{figure}[h!]
                \centering
                \begin{tabular}{||c|c||}
                \hline
                \verb+ POLINIZADORES + & \verb+ PLANTAS  + \\ \hline
                \includegraphics[width=4.8cm,height=4.2cm]{imagenes/prog10_03.png} & \includegraphics[width=4.8cm,height=4.2cm]{imagenes/prog10_04.png}  \\  
                \hline
                \includegraphics[width=4.8cm,height=4.2cm]{imagenes/prog10_01.png} & \includegraphics[width=4.8cm,height=4.2cm]{imagenes/prog10_02.png} \\ 
                \hline
                \end{tabular}
                \caption{Estado estacionario del sistema (\ref{eq:eq1numre}) con $D_1=10$.}
                \label{pol:fig6} 
                \end{figure}  
                  
                
                
                
                      
                      
\clearpage                
                
\newpage                
               
               
               \subsection{Problema no lineal: Estado estacionario de Plantas-Herb\'{i}voros}
               
               En esta secci\'{o}n vamos a estudiar el siguiente sistema de ecuaciones                                                                                      
                \begin{eqnarray}
                \label{par:phnumre}  
                       p \left( 1-\displaystyle\frac{p}{k} \right) - \displaystyle\frac{ph}{1+p} & = & 0,  \\
                       D_2 div \left[ f_2(p) \bigtriangledown h \right] - \alpha \beta h + \beta  \displaystyle\frac{ph}{1+p} & = & 0 ,   \nonumber
                \end{eqnarray}          
                con condiciones de Dirichlet no homog\'{e}neas, i.e.
                \begin{equation}
                 p(\vec{x}) = p_f, \hspace{0.2cm} h(\vec{x}) = h_f, \hspace{0.5cm}  \forall   \vec{x} \in \partial \Omega,
                \end{equation}
                donde $p = p (\vec{x})$ y $h=h(\vec{x})$ representan la densidad de las plantas y los herb\'{i}voros,
                respectivamente, en el punto $ \vec{x} \in \Omega$; $p_f$ y $h_f$ son constantes positivas. 
                N\'{o}tese que el sistema (\ref{par:phnumre}) puede ser un sistema degenerado, eso depender\'{a} 
                de los valores de $p$.                             
                
                Este sistema describe el estado estacionario de la interacci\'{o}n entre la poblaci\'{o}n
                de las plantas y los  herb\'{i}voros.             
                
                Si $0<\alpha<1$, entonces el sistema (\ref{par:phnumre}) tiene tres estados 
                estacionarios homog\'{e}neos: $(0,0)$; $(k,0)$ y $(\tilde{p},\tilde{h})$,  
                donde                  
                \begin{equation*}
                      \tilde{p}=\displaystyle\frac{\alpha}{1-\alpha}, \hspace*{1cm} \tilde{h}=(1+\tilde{p}) \left(1-\displaystyle\frac{\tilde{p}}{k}\right).
                \end{equation*}               

                Con el prop\'{o}sito de buscar soluciones no constantes para el sistema (\ref{par:phnumre}) 
                consideremos que $p \neq 0$, as\'{i} de la primera ecuaci\'{o}n de este sistema, tenemos que
                \begin{equation}
                \label{eq:solep}  
                           h = ( 1+p ) \left( 1-\displaystyle\frac{p}{k} \right), 
                \end{equation} 
                lo cual nos est\'{a} diciendo que la distribuci\'{o}n final de la poblaci\'{o}n de los herb\'{i}voros
                est\'{a} relacionada de manera no lineal con la distribuci\'{o}n final de la poblaci\'{o}n de las 
                plantas. 

                De hecho esta relaci\'{o}n tambi\'{e}n nos est\'{a} diciendo que si $p \equiv p(\vec{x}) $ 
                tiene un m\'{a}ximo en la posici\'{o}n $\vec{x}_1$, entonces $h \equiv h(\vec{x})$
                tendr\'{a} un m\'{i}nimo en esa misma posici\'{o}n. De manera an\'{a}loga sucede con
                el m\'{i}nimo, es decir, si $p \equiv p(\vec{x}) $ tiene un m\'{i}nimo en $\vec{x}_2$,
                entonces $h \equiv h(\vec{x})$ tendr\'{a} un m\'{a}ximo en esa misma posici\'{o}n.
                 
                Por otro lado la relaci\'{o}n anterior nos permite simplificar el sistema (\ref{eq:estph}) 
                como                
                \begin{equation*}                
                       D_2 div \left[ f_2(p) \bigtriangledown h \right] - \alpha \beta ( 1+p ) \left( 1-\displaystyle\frac{p}{k} \right) + \beta  p \left( 1-\displaystyle\frac{p}{k} \right)  =  0,
                \end{equation*}
                o equivalentemente
                \begin{equation}  
                \label{eq:redph}
                      D_2 div \left[ f_2(p) \bigtriangledown h \right] = \beta \left( 1-\displaystyle\frac{p}{k} \right) \left[  \alpha  +  ( \alpha-1 ) p  \right] ,
                \end{equation}
                donde $h=( 1+p ) \left( 1-\frac{p}{k} \right)$ y $k$, $\alpha$ y $\beta$ son par\'{a}metros positivos.
   
                Por lo que de aqu\'{i} en adelante s\'{o}lo nos enfocaremos en estudiar las propiedades
                cualitativas de la ecuaci\'{o}n diferencial (\ref{eq:redph}).       
               

               
               
               
               
                
                
                
                
               
            
                
 
               
               
                

               \section{Coordenadas de los dominios}
               Las coordenadas cartesianas de los diferentes dominios $\Omega$,
               en el orden en que fueron apareciendo a partir de la secci\'{o}n 
               \ref{Resultados}, se describen a continuaci\'{o}n.
               
               Las coordenadas de los v\'{e}rtices del tri\'{a}ngulo son:
               \begin{equation*}
                     (1,1); (13,1); \text{ y } (7,12.25).
               \end{equation*}

               Las coordenadas de los v\'{e}rtices del pent\'{a}gono son:
               \begin{equation*}
                     (1.1,8); (7,12.25); (12.8,8); (10.5,1)  \text{ y } (3.5,1).
               \end{equation*}
               
               Las coordenadas de los v\'{e}rtices de la estrella son:
               \begin{eqnarray*}
                     (1.1,8); (5.6,8); (7,12.25); (8.4,8); (12.8,8);  \\
                     (9.2,5.4); (10.5,1); (7,3.6); (3.5,1) \text{ y } (4.8,5.4).
               \end{eqnarray*}

                               
                               
                
                \subsection{Observaciones}                                  
                
                Las soluciones que se obtuvieron con {\it Matlab} y {\it FlexPDE} 
                para ambos problemas son cualitativamente similares, de hecho el valor m\'{a}ximo 
                que alcanza cada una de las soluciones obtenidas tanto con {\it Matlab} como
                con {\it FlexPDE} son aproximadamente los mismos.      
                
                Es importante mencionar que los resultados que se obtuvieron al resolver los 
                mismos problemas sobre $\underline{\Omega}$ son muy parecidos a los que se 
                obtuvieron para $\overline {\Omega}$, los cuales no se incluyeron aqu\'{i} para
                no hacer hacer m\'{a}s largo el documento   

                
                
                %\begin{figure}[h!]
                %\centering                
                %\begin{tabular}{||c | c||}     
                %\hline                                                
                %\includegraphics[width=6.0cm,height=5.0cm]{metodo2/solAproxSurf1.jpg} & %%\includegraphics[width=6.0cm,height=5.0cm]{metodo2/solExacSurf1.jpg} \\                  
                %\hline
                %\includegraphics[width=6.0cm,height=5.0cm]{metodo2/solAproxMesh1.jpg} & \includegraphics[width=6.0cm,height=5.0cm]{metodo2/solExacMesh1.jpg} \\                  
                %\hline
                %\end{tabular}
                %\caption{Soluci\'{o}n num\'{e}rica de la ecuaci\'{o}n (\ref{Parabola:eq})
                %         sobre $\overline {\Omega}$ y $\underline{\Omega}$, respectivamente.}
                %\label{fig:ParabolaSol}
                %\end{figure}               
                
                Hasta este momento s\'{o}lo hemos establecido como construir una 
                sucesi\'{o}n de soluciones y la cual queremos que converga 
                a la soluci\'{o}n del problema. De hecho, esta sucesi\'{o}n de 
                soluciones la obtenemos a trav\'{e}s de aplicar de manera 
                adecuada el m\'{e}todo de diferencias finitas a una sucesi\'{o}n 
                de dominios que aproximan a la regi\'{o}n irregular. M\'{a}s 
                a\'{u}n, la sucesi\'{o}n de dominios y de soluciones las vamos
                a generar mediante un algoritmo. 
                
                %La convergencia en cada direccion es diferente y por lo tanto el 
                %la eleccion de los deltas debe de ser diferente.
                
                %Para obtener la misma velocidad de convergencia en ambas direcciones
                %se requiere de una delta mas pequeña en la direccion de convergencia
                %más lenta. Y una delta mas grnade en la direccion de convergencia
                %mas rapida.
                
                %Recuerda que la delta entre mas pequeña converge mas rapido.
                

                
                %Dominio condicionalmente extendible y contraible
                %Dominio completamente extendible y contraible
                
                

